SG-Reg: Generalizable and Efficient Scene Graph Registration

This paper addresses the challenges of registering two rigid semantic scene graphs, an essential capability when an autonomous agent needs to register its map against a remote agent, or against a prior map. The hand-crafted descriptors in classical semantic-aided registration, or the ground-truth annotation reliance in learning-based scene graph registration, impede their application in practical real-world environments. To address the challenges, we design a scene graph network to encode multiple modalities of semantic nodes: open-set semantic feature, local topology with spatial awareness, and shape feature. These modalities are fused to create compact semantic node features. The matching layers then search for correspondences in a coarse-to-fine manner. In the back-end, we employ a robust pose estimator to decide transformation according to the correspondences. We manage to maintain a sparse and hierarchical scene representation. Our approach demands fewer GPU resources and fewer communication bandwidth in multi-agent tasks. Moreover, we design a new data generation approach using vision foundation models and a semantic mapping module to reconstruct semantic scene graphs. It differs significantly from previous works, which rely on ground-truth semantic annotations to generate data. We validate our method in a two-agent SLAM benchmark. It significantly outperforms the hand-crafted baseline in terms of registration success rate. Compared to visual loop closure networks, our method achieves a slightly higher registration recall while requiring only 52 KB of communication bandwidth for each query frame. Code available at: \href{http://github.com/HKUST-Aerial-Robotics/SG-Reg}{http://github.com/HKUST-Aerial-Robotics/SG-Reg}.

==> experiments/ablation_data.tex <==
\subsubsection{Ablation study on training data}\label{sec:3rscan_gt}
This section evaluates how the training data influences the final performance. We train SG-PGM and our method using 3RScan-GT data and test all models in 3RScan-Mapping. Their performance are compared with the model trained using ScanNet-Mapping.
% We follow previous works\cite{sarkar2023sgaligner}\cite{xie2024sgpgm} to generate scene graph data from 3RScan with ground-truth annotations. We denote their training data as 3RScan-GT.  Our training data is denoted as ScanNet-Mapping.
\begin{figure}[h]
    \centering
    \begin{subfigure}[h]{0.47\columnwidth}
        \includegraphics[width=\columnwidth]{fig/rio/sgalign_data.png}
        \caption{3RScan-GT}
    \end{subfigure}
   \begin{subfigure}[h]{0.5\columnwidth}
        \includegraphics[width=\columnwidth]{fig/rio/scannet_mapping3.png}
        \caption{ScanNet-Mapping}
    \end{subfigure}
    \caption{Visualize the training data. (a) 3RScan-GT generated by SGAligner. (b) ScanNet-Mapping reconstructed via semantic mapping\cite{liu2024fmfusion}. 
    % Two nearby couches are falsely integrated as one couch.
    }
    \label{fig:sgalign_data}
\end{figure}

As the example shown in Fig. \ref{fig:sgalign_data}(a), 3RScan-GT provides a clearly segmented point cloud. Each semantic node is reconstructed completely without effects from occlusion. It is annotated with a ground-truth semantic label. In each re-scan, semantic labels are guaranteed to be consistent with the labels from the previous scan. On the other hand, point cloud segmentation in ScanNet-Mapping is incorporated with significant variance, as shown in Fig. \ref{fig:sgalign_data}(b). Some of the chairs are under-segmented or partially reconstructed due to occlusion. Point cloud from the glass door is noisy due to the depth noise when it is observed by the RGB-D camera. Besides, the semantic label of each node can be inconsistent when re-scan it in a new SLAM session.

\begin{table}[h]
    \centering
    \begin{tabular}{c|c c c c c}
        \hline
         % \multirow{2}{*}{Training Data} & \multicolumn{3}{c}{3RScan-SLAM}\\
         & Training Data & NR(\%) & NP(\%)& IR(\%) & RR(\%) \\
         \hline
         \multirow{2}{*}{SG-PGM} & 3RScan-GT & $39.2$ & $25.8$ &7.8 & 38.3 \\
         & ScanNet-Mapping & $\mathbf{50.7}$ & $\mathbf{27.0}$ & $\mathbf{8.3}$ & $\mathbf{51.1}$ \\ % no bert
         % TP: 136 378 202 261
         \hline
         \multirow{2}{*}{Ours} & 3RScan-GT & $26.4$ & ${32.3}$ & 6.1 & 42.6 \\
         & ScanNet-Mapping & $\mathbf{73.2}$ & $\mathbf{35.3}$ & $\mathbf{6.4}$ & $\mathbf{78.7}$ \\
        \hline
    \end{tabular}
    \caption{Ablation study on the training data. We evaluate the performance in 3RScan-Mapping data.}
    \label{tab:traindata}
\end{table}

As shown in Table. \ref{tab:traindata}, our network and SG-PGM that are trained with 3RScan-GT perform poorer than training them with ScanNet-Mapping data. Suffering from the domain gap, both of them perform poorly in matching the real-world integrated scene graphs.

It demonstrates that the training data is critical in maintaining a generalizable scene graph matching network.
The real-world integrated scene graph contains significant variances in high-dimensional feature space. Such variance can not be easily imitated through data augmentation. The best way is to generate data from the same mapping pipeline as us. So, the training data is incorporated with similar variances, and it enables the network to learn it in the training process. \lchcomment{maybe in more academic explanation? data bias?}

==> experiments/ablation_icp.tex <==
\subsubsection{Ablation study on ICP refinement}

As the mainstream method for point cloud registration, ICP can provide high-precision alignment results, but it heavily relies on the initial position. 
% On the contrary, our method and the two baselines can handle larger initial disparities but can hardly achieve a comparable high-precision result as ICP. Therefore, these methods can serve as pre-order methods, providing an optimized initial value for ICP. In this ablation study, we incorporate ICP refinement into all methods. 
As shown in Table. \ref{tab:icp_refine}, the baseline methods and our method can serve as pre-order methods, providing an optimized initial value for ICP.
We report the results from ICP refinement to show the upper bounds of each registration method.

\begin{table}[ht]
    \centering
    \begin{tabular}{c c c c}
        \toprule
         & GeoTransformer & SG-PGM & \textbf{SG-Reg}  \\
        \hline
        % G3Reg & $53.2(+0.0)$ & $57.4(+6.3)$ & $\mathbf{85.1}$(N/A)\\
        % {Without ICP} & RR(\%) & {75.9} & 39.0 & 76.0 \\
        % & RMSE(m) & {0.069} & \textbf{0.086} & 0.108\\
        % \hline
        RR(\%) & {91.0}(+16.8) & 54.0(+19.0) & \textbf{92.0}(+\revise{13.0}) \\
        % & RMSE(m) & 0.074 & 0.066 & {0.061} \\
        \bottomrule
    \end{tabular}
    \caption{Registration boosted by ICP refinement.}
    \label{tab:icp_refine}\vspace{-0.5cm}
\end{table}


==> experiments/ablation_point_match.tex <==
\subsubsection{Ablation study on point match}
In this ablation study, we incorporate the superpoint and its encoder from GeoTransformer into our method. The matched node guides the matches between super points. Then, matched the superpoint guide he matches between point clouds.

\begin{figure}[h]
    \centering
    \begin{subfigure}[h]{0.47\columnwidth}
        \includegraphics[width=\columnwidth]{fig/todo.png}
        \caption{SG-PGM}
    \end{subfigure}
    \begin{subfigure}[h]{0.47\columnwidth}
        \includegraphics[width=\columnwidth]{fig/todo.png}
        \caption{Ours}
    \end{subfigure}
    \caption{Point match result at a sub-volume in 3RScan. The number of true positive nodes and true positive points are annotated at the top right corner.}
    \label{fig:pt-match}
\end{figure}

Our point features are primarily similar since both of us use the pre-trained KPConv backbone. Therefore, we believe that we perform differently because of our matching strategies. 
On the other hand, we search matches in two layers: Node-Point.

Although we can also implement three layers of matches to achieve a higher IR, we keep our matching strategy for two reasons. Firstly, we use a robust pose estimator which can tolerate a higher outlier ratio\cite{qiao2024g3reg}. Our registration recall is already higher than all the baseline methods we compared. Secondly, the geometric transformer for the super-point consumes a large amount of GPU memory. It hurts the efficiency of our method.

==> experiments/preception_field.tex <==
\subsubsection{Evaluate Perception Field}
We design another ablation study to explore the influence of the perception field. Our method constructs edges between nearby semantic nodes, as shown in Fig. \ref{fig:explicit_sg}. Each node is aware of its local topology in the scene graph. In the ablation study, we connect each node with all of the other nodes in the scene graph and denote their edges as a global edge set. It is similar to SuperGlue\cite{sarlin20superglue} in that the self-attention GNN aggregates an image feature with all of the other image features. The global edge set incorporates a large perception field into the node features and learns a global topology feature in the graph embedding.
With the global edge set, we train and evaluate the three GNN backbones. The shape feature is not fused in this ablation study.

\begin{table}[h]
    \centering
    \begin{tabular}{c c c}
        \hline
        \hline      
        & Node Rec.(\%) &Node  Prec.(\%) \\
        \hline
        RPE GAT & 74.3 (-0.7) & 51.5 (-1.2) \\
        Geometric Transformer & Not Converge & Not Converge \\
        Triplet-boosted GNN (\textbf{Ours}) & 77.2 (+0.4) & 52.2 (-5.3) \\
        \hline
        \hline
    \end{tabular}
    \caption{The performances after all the edges are incorporated in constructing the scene graph. We highlight the relative change compared with the results in Table. \ref{tab:scannet}.}\label{tab:eval-edges}\vspace{-0.3cm}
\end{table}
As shown in Table \ref{tab:eval-edges}, we find that a larger perception field affects the node precision of all the investigated GNN methods. We believe there are two possible reasons. Firstly, many of the scene graphs have a low overlap volume. So, their global edge sets are largely different. Aggregating using the global edge set makes the graph matching less accurate. Secondly, the scene graph reconstructed from semantic mapping involves a significant variance. A large perception field magnifies the effects of the variances. 

==> experiments/semantic_generalize.tex <==
\subsubsection{Semantic Generalization}
Our method can match the semantic objects it has never seen during the training. For example, the \textit{elevator} shown in Fig.\ref{fig1} is matched correctly, although the ScanNet training data has not provided any scene with a \textit{elevator}. Our method can be generalized in new semantic categories for two reasons. Firstly, we encode the semantic label by Bert. So, our network can read new semantic labels. Secondly, the triplet-boosted GNN learns a general spatial topology between semantic nodes. We have not designed any hand-craft rules to construct the descriptor. So, the learned topology is not limited by the semantic labels.


==> experiments/shape_encoder.tex <==
\subsubsection{Discuss Shape Encoder}
\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c}
        \hline
         & Require Concatenate & \multirow{2}{*}{Without Concatenate} \\
         & (Current KPConv)& \\
         \hline
        Fine-level Message & $\mathcal{Y}^A$ & ${\varffeat}^A $ \\
        Average Bandwidth & ? & ?\\
        Shape Encoder Input & $\{\varyy^A, \varyy^{R_i}\}_i$ & $\varyy^A$ \\
        Shape Enc. Time & $\approx 400$ ms & ?\\
         \hline
    \end{tabular}
    \caption{Communication bandwidth and shape encoder efficiency influenced by point cloud backbone. Notice that the point cloud number $\vert \varyy^A \vert$ is significantly larger than the nodes number $\vert \varffeat^A \vert$. And broadcast $\varyy^A$ cost larger data bandwidth. \lchcomment{todo}}
    \label{tab:shape_limit}
\end{table}

In our current shape encoder, we use KPConv\cite{thomas2019kpconv} backbone that is trained by GeoTransformer. It is trained in a point cloud registration task and generalizes well in our experiment. KPConv requires the two point cloud be concatenated to run, because it incorporates multiple group normalization layers during the encoding. The group normalization layers implicit incorporate correlation between the embedding of the point cloud pair. And it guarantees the point cloud matching performance. However, the concatenate operation affects the communication bandwidth and scale-up ability of SG-Reg.
As shown in Table. \ref{tab:shape_limit}, an agent A has to broadcast its dense points $\varyy^A$ in its fine-level message. Compare with broadcasting the encoded shape features $\varffeat^A$, it costs larger data bandwidth. Besides, an agent has to encode the point cloud with its counterpart from each remote agent $\varyy^{R_i}$. For example, if there are two remote agents, agent A has to run the shape encoder twice in each loop frames. The repeated encoding cost large computing resources. And it seriously limits SG-Reg be scaled up to a larger amount of autonomous agents.
